Circuits and Formulas for Datalog over Semirings

In this paper, we study circuits and formulas for provenance polynomials of Datalog programs. We ask the following question: given an absorptive semiring and a fact of a Datalog program, what is the optimal depth and size of a circuit/formula that computes its provenance polynomial? We focus on absorptive semirings as these guarantee the existence of a polynomial-size circuit. Our main result is a dichotomy for several classes of Datalog programs on whether they admit a formula of polynomial size or not. We achieve this result by showing that for these Datalog programs the optimal circuit depth is either $\Theta(\log m)$ or $\Theta(\log^2 m)$, where $m$ is the input size. We also show that for Datalog programs with the polynomial fringe property, we can always construct low-depth circuits of size $O(\log^2 m)$. Finally, we give characterizations of when Datalog programs are bounded over more general semirings.

==> lower_bound.tex <==
%\section{Lower Bounds}
\blue{In this section, we prove several circuit depth lower bounds for unbounded datalog program. All Datalog programs will be over $\bB$ unless stated otherwise. By Proposition~\ref{prop:positive_semiring}, all lower bounds results over $\bB$ transfer easily to any positive semiring.
}



\subsection{Lower Bounds for Monadic Linear Datalog Program}
In this section, we prove $\Omega(\log^2 n)$ circuit depth lower bound for any unbounded monadic linear Datalog program over $\bB$. This implies a super-polynomial formula size lower bound for those programs over any positive semiring. 

We start with some definitions~\cite{CosmadakisGKV88}. Given a set of atoms $F$, the {\em variable graph} for $F$ is an undirected graph $G_F = (V,E)$ where $V$ is the set of variables appears in $F$ and two variables are connected by an edge if and only if they both appear in one atom in $F$. A rule $r$ in a monadic linear Datalog program is of the form $Q_1(X):- A, Q_2(Y)$ where $Q_i$'s are IDBs and $A$ is the set of EDBs in the rule; $Q_2$ could be potentially absent, in which case the rule is an initialization rule rather than a recursive rule.  We assume $X \neq Y$ in all recursive rules. We say that a rule $r$ is {\em connected} if $G_A$ is a connected graph and $X, Y$ are vertices in $G_A$. A program is called {\em connected} if every rule is connected. 

Given a linear monadic program $\Pi$ with recursive bodies $\{A_1, \dots, A_m\}$ and initialization bodies $\{B_1, \dots, B_n\}$, we consider the expansions of $\Pi$ into $\CQ$s, called {\em $Q$-expansions}, that sequentially apply some recursive rules and finish with a initialization rule~\cite{CosmadakisGKV88}, in the spirit of Theorem~\ref{thm:bound:idem}. Formally, the {\em recursive alphabet} $\Sigma_{\Pi, r}$ is the set $\{a_1, \ldots, a_m\}$, and {\em initialization alphabet} $\Sigma_{\Pi, i}$ is the set $\{b_1, \ldots, b_n\}$. The {\em alphabet} $\Sigma_{\Pi}$ is the union of $\Sigma_{\Pi, r}$ and $\Sigma_{\Pi, i}$. Then, the set of $Q$-expansions of the program $\Pi$ can be viewed as a language over $\Sigma_{\Pi}$; we denote this language as $\operatorname{expand}(\Pi, Q)$. Furthermore, let $C$ be a $\CQ$ denoted by a word of $(\Sigma_{\Pi, r})^*$ or a word of $\left(\Sigma_{\Pi, r}\right)^*\left(\Sigma_{\Pi, i}\right)$. We say that $C$ is {\em $Q$-accepted} by $\Pi$, if there is some $Q$-expansion $C_i$ such that there exists a homomorphism from $C_i$ to $C$, which implies the result of $C$ is contained in $C_i$ over $\bB$~\cite{ChandraM77}. Let $\operatorname{accept}(\Pi, Q)$ be the language over alphabet $\Sigma_{\Pi}$ consisting of the word which denote conjunctive queries $Q$-accepted by $\Pi$. The language $\operatorname{notaccept}(\Pi, Q)$ is the complement of accept $(\Pi, Q)$ over $(\Sigma_{\Pi}^*)$ . Note that $\operatorname{expand}(\Pi, Q) \subseteq \operatorname{accept}(\Pi, Q)$.

The following result is proved in~\cite{CosmadakisGKV88} that characterizes the boundedness of a linear connected monadic program.

\begin{theorem}[Cosmadakis, Gaifman, Kanellakis \& Vardi, 88']
    Let $\Pi$ be a linear connected monadic program and let $Q$ be an IDB predicate of $\Pi$. Then, $Q$ is unbounded in $\Pi$ if and only if for every $k>0$, there is a word $w$ in $\operatorname{expand}(\Pi, Q)$ such that $|w|>k$ and the prefix of $w$ of length $k$ is in $\operatorname{notaccept}(\Pi, Q)$.
\end{theorem}

We shall also make use of the following proposition proved in~\cite{CosmadakisGKV88}.

\begin{proposition}
    Both the language $\operatorname{expand}(\Pi, Q)$ and $\operatorname{notaccept}(\Pi, Q)$ are regular.
\end{proposition}

We are now ready to prove that any unbounded monadic linear program admits a $\Omega(\log^2 n)$ circuit depth lower bound over $\bB$. The main idea is to encode each edge between two layers by canonical database of the expansions instead of as a sequence of edges in the case of $\CFG$.

\begin{theorem}
    If an IDB $Q$ in a connected monadic linear datalog program $\Pi$ is unbounded, then there exists a set of EDBs and a tuple $t$ in $Q$ such that the circuit for the provenance polynomial of $t$ over $\bB$ has depth $\Omega(\log ^2n)$.
\end{theorem}
\begin{proof}
    % We call a recursive rule {\em unessential} if it is of the form $Q_1(X):-A, Q_2(X)$, i.e.\ the variable inside the IDB atoms are the same. We claim that $Q$ in program $\Pi$ is unbounded if and only if $Q$ is unbounded when we remove all unessential rules from $\Pi$. Indeed, all such  
    We reduce from $\TC$ to $\Pi$ where $Q$ is the designated output IDB. Suppose $G$ is the input $(\ell, n)$-layered directed graph and $s, t$ are the distinguished vertices. Since $\operatorname{notaccept}(\Pi, Q)$ is a regular language, its complement $\operatorname{accept}(\Pi, Q)$ is also a regular language. By the pumping lemma, there exists a word $xyz$ in $\operatorname{accept}(\Pi,Q)$ such that $xy^iz$ lies in $\operatorname{accept}(\Pi,Q)$ for any integer $i$. 

    We construct the EDBs as follows:
    \begin{enumerate}
        \item Let \austen{consideratum: Backwards of $xyz$; want all initialization rules of $Q$ to result in a single $s$, while encoding each edge by the canonical database of the expansion.}
    \end{enumerate} 
\end{proof}
\austen{Connected and disconnected}

\austen{How expansions related to strings; turn expansions into canonical database}

\austen{Discuss where the proof breaks when the program is unbounded.}

\austen{Generalize to the Yannnakakis etc.. form for binary; that's undecidable for boundedness ?}

\austen{Mention the seek of pumping lemma for datalog}

\subsection{Linear Sirups}
\begin{theorem}
    If an IDB $R$ in a linear Sirups $\Pi$ is unbounded, then there exists a set of EDBs and a tuple $t$ in $R$ such that the circuit for the provenance polynomial of $t$ over positive semiring has depth $\Omega(\log ^2n)$.
\end{theorem}
\begin{proof}
        Observe that in previous lower bounds, the essence is to construct a sequence of strings such that we can encode the $st$-reachability for layered directed graphs.  \austen{Discuss the ``for all'' in pumping lemma and how to prove result by relaxing to ``there exists''.}
\end{proof}
    
